Information Theory of DNA Shotgun Sequencing

DNA sequencing is the basic workhorse of modern day biology and medicine. Shotgun sequencing is the dominant technique used: many randomly located short fragments called reads are extracted from the DNA sequence, and these reads are assembled to reconstruct the original sequence. A basic question is: given a sequencing technology and the statistics of the DNA sequence, what is the minimum number of reads required for reliable reconstruction? This number provides a fundamental limit to the performance of {\em any} assembly algorithm. For a simple statistical model of the DNA sequence and the read process, we show that the answer admits a critical phenomena in the asymptotic limit of long DNA sequences: if the read length is below a threshold, reconstruction is impossible no matter how many reads are observed, and if the read length is above the threshold, having enough reads to cover the DNA sequence is sufficient to reconstruct. The threshold is computed in terms of the Renyi entropy rate of the DNA sequence. We also study the impact of noise in the read process on the performance.

==> achievability_intuitive.tex <==
%% new commands


%\newcommand{\pe}{P_\text{error}}

\section{Optimal Algorithm}
\label{sec: achieve}

Our framework allows to evaluate the minimum number of reads required for various concrete reconstruction algorithms, allowing to compare their performance. We begin by deriving the performance of a simple sequential algorithm, which is seen to be suboptimal. This leads naturally to an optimal greedy algorithm, whose performance (perhaps surprisingly) matches the lower bounds of Section~\ref{sec:lower}. The reasoning in this section is heuristic in nature; a rigorous proof of optimality for the greedy algorithm is deferred to Section~\ref{sec:proofs}. 


\subsection{Sequential algorithm}

The paper of Lander and Waterman \cite{LW88} implicitly suggests an algorithm for assembly. They assume that there is a positive integer $T$ such that an overlap of $T$ bases between two reads can be correctly detected, with few false positives. 
If $T$ is the minimum overlap between two adjacent reads, and indeed $T$ is sufficiently large that with high probability there are no false positives, merging reads sequentially to grow a single fragment correctly assembles the genome. In more detail, we have 
\\
\\
 \emph{Sequential Algorithm:}
\begin{enumerate}
\item Let the current fragment consist of an arbitrary read
\item Extend the current fragment sequentially to the right by merging a read with highest overlap
\item Repeat Step~2 until all reads have been merged 
\end{enumerate}
%To ensure correctness of the algorithm, one must only verify that $T$ is indeed large enough to rule out false positives, and that the minimum overlap is $T$. 
%However, \cite{LW88} did not specify a value for $T$; our stochastic sequence model allows us to do so. 


The salient question is how many reads does this algorithm require.

\begin{theorem}\label{t:sequentialRate}
Fix $\bar{L}=L/\ln G$. The minimum number of reads required by the sequential algorithm satisfies $G/N=C_\text{seq}$, where $C_\text{seq}$ is given by 
\begin{enumerate}
\item If $\bar{L}<2/H_2(\mathbf{p})$ then $C_{\text{seq}} = 0$.
\item If $\bar{L}>2/H_2(\mathbf{p})$ then $C_{\text{seq}} = \bar{L}/2$
\end{enumerate}
\end{theorem}

In the rest of this subsection we heuristically prove Theorem~\ref{t:sequentialRate}, simultaneously illustrating the general framework and obtaining an understanding of the sequential algorithm.
We begin by defining a probabilistic event $\calA$ capturing the success of the algorithm, then estimate the probability of error $\P(\calA^c)=\pe$ for a fixed choice of parameters $G, \bar{L},$ and $c=\frac{G}N$, and finally deduce the maximum value of $c$ such that $\pe$ approaches zero as $G\to \infty$. 

The event $\calA$ that the algorithm is successful can be written in terms of events denoting successful merging for each read. Recall that $\ph_{ij}$ denotes the physical overlap between reads $R_i$ and $R_j$, $\ph_i$ is the physical overlap between $R_i$ and $R_{i+1}$, and $w_{ij}$ denotes the maximum length suffix of $R_i$ and prefix of $R_j$ which are equal. Starting with $R_1$ (for convenience), the sequential algorithm successfully merges $R_{i+1}$, the successor to $R_i$, if the physical overlap between $R_i$ and $R_{i+1}$ is greater than the putative overlap $w_{ij}$ between $R_i$ and all reads $R_j$, $j> i$; let $\calA_i =\{\ph_i>\max_{j>i+1}w_{ij} \}$ denote this event.
Note that only reads $R_j$ with $j>i+1$ can cause an error, since reads $R_1,\dots, R_i$ have already been merged. The event that the sequential algorithm succeeds is thus $\calA = \cap_i \calA_i$.

Our goal is to estimate 
\begin{equation}\label{e:unionA}
\pe=\P(\calA^c)\approx \sum_{i=1}^N \calA_i^c\,,
\end{equation} where the approximation assumes the union bound on probabilities is tight.
Now for $i\leq N/2$, conditioning on an overlap of size $\ell$ we get
\begin{equation}\label{e:conditioning}
\P(\calA_i^c|\ph_i=\ell) = \P( \ell\leq\max_{j>i+1}w_{ij}) \approx \sum_{j>i+1} \P(\ell\leq w_{ij})%\approx \frac{N}2 \P(\ell\leq w_{ij}) = 
\approx N e^{-\ell H_2(\p)}\,,
\end{equation}
where the last step is by Lemma~\ref{l:matchProb},
and only holds if $R_i$ and $R_j$ are disjoint, which we suppose to be approximately true since this holds for most pairs of reads.

Combining \eqref{e:unionA} and \eqref{e:conditioning}, the total probability of error is thus
\begin{equation}\label{e:SeqProbError}
\pe \approx \sum_{i=1}^N \sum_{\ell=0}^L \P(\calA_i^c|\ph_i=\ell)\P(\ph_i=\ell) \approx N^2 \sum_{\ell=0}^L  e^{-\ell H_2(\p)}\P(\ph_i=\ell)\,.
\end{equation} In order to evaluate the above probability of error, we find $f_N(\ell):=\P(\ph_i=\ell)$, the probability distribution of overlaps. 
The $i$th overlap is $\ph_i=(L-T_i)^+$, where $T_i\sim \Exp{\lam}$ is the $i$th inter-arrival time, so we have that
\begin{equation}
f_N(\ell)=\left(\lam e^{-\lam(L-\ell)}+e^{-\lam L}\de(\ell)\right)\approx e^{-\lam(L-\ell)} \,.
\end{equation}
Here $\de(x)$ is the Dirac-delta function.
%Consequently, the empirical CDF is given by
%\begin{align}
%F_N(\ell)=\int_0^\ell f_N(k)dk=e^{-\lam L}+e^{-\lam(L-k)}|_{k=0}^\ell&=e^{-\lam(L-\ell)}\,.
%\end{align}

Plugging into \eqref{e:SeqProbError}, we have our desired estimate
\begin{equation}
\pe \approx N^2 \sum_{\ell=0}^L f_N(\ell)e^{-\ell H_2(\p)}%\approx N^2 \sum_{\ell=0}^L F_N(\ell)e^{-\ell H_2(\p) }=
\approx N^2 \sum_{\ell=0}^L e^{-\lam(L-\ell)} e^{-\ell H_2(\p)} \,.
\end{equation}
Such an exponential sum is dominated by either the first or last term. If $\bar{L}> \frac{2}{H_2(\p)}$, as we know is necessary by Section~\ref{sec:lower}, then the $\ell=L$ term becomes negligible. Requiring the $\ell=0$ term to be small implies $$c=\frac GN=\lambda\inv < \frac{\bar{L}}2\,.$$ 

The minimum $N$ required is a factor two larger than the necessary condition of Section~\ref{sec:lower} in the coverage-limited regime. What is impeding the sequential algorithm? As observed in Lemma~\ref{l:matchProb}, the likelihood of error is quite small when considering a read with high overlap to its successor. The bottleneck is therefore in determining the successors of reads with relatively little overlap. 

This difficulty can be circumvented by first merging the ``easy" reads, i.e. those with large overlap to the subsequent read. As progressively smaller overlaps are encountered, fewer potentially confusing reads remain. In the final step only a pair of reads remain, and these can be correctly merged even if their overlap is small. This rule---merge reads with the highest overlap first---prescribes the greedy algorithm described in the next subsection.




\subsection{Greedy Algorithm}

The greedy algorithm is given as follows.
\\

 \emph{Greedy Algorithm:}
\begin{enumerate}
\item Find two fragments with largest overlap
\item Merge the two selected fragments
\item Repeat until only one fragment remains
\end{enumerate}
The greedy algorithm turns out to be optimal, i.e. it achieves capacity as described in Theorem~\ref{t:mainCapacity}.

The performance analysis is similar to that for the sequential algorithm above, with one crucial difference: 
When considering a read $R_i$, all reads $R_j$ with overlap $\ph_j>\ph_i$ have \emph{already} been merged to their successors. Thus, read $R_i$ is correctly merged to $R_{i+1}$ if the event $\calA_i =\{\ph_i>\max_{j:\ph_j\leq \ph_i}w_{ij} \}$ occurs, meaning that all reads $R_j$ which still remain do not appear to have higher overlap with $R_i$ than the true successor $R_{i+1}$. The intersection $\calA = \cap_i \calA_i$ captures the successful assembly of the DNA sequence, and as before we wish to estimate $\P(\calA^c)\approx \sum_i \P(\calA_i^c)$. 

Conditioning gives
\begin{equation}\label{e:conditioning2}
\P(\calA_i^c|\ph_i=\ell) = \P( \ell\leq\max_{j:\ph_j\leq \ell}w_{ij}) \approx \sum_{j:\ph_j\leq \ell}\P(\ell\leq w_{ij})%\approx \frac{N}2 \P(\ell\leq w_{ij}) = 
\approx (Nf_N(\ell)) e^{-\ell H_2(\p)}\,,
\end{equation}
where the last step follows because there are approximately $Nf_N(\ell)$ reads with $\ph_j\leq \ell$. The difference between the greedy and sequential algorithms is highlighted when comparing~\eqref{e:conditioning2} with~\eqref{e:conditioning}.

The total probability of error is, by \eqref{e:conditioning2} and the definition of $f_N(\ell)=\P(\ph_i=\ell)$,
\begin{equation}\begin{split}\label{e:GreedyProbError}
\pe   \approx \sum_{i=1}^N \sum_{\ell=0}^L \P(\calA_i^c|\ph_i=\ell)\P(\ph_i=\ell) &= N^2 \sum_{\ell=0}^L (f_N(\ell)\big)^2e^{-\ell H_2(\p) }
\\ &= N^2 \sum_{\ell=0}^L e^{-2\lam(L-\ell)} e^{-\ell H_2(\p)} 
\,.
\end{split}
\end{equation}
The only difference in $\pe$ compared to the sequential algorithm \eqref{e:SeqProbError} is a factor two in front of $\lam$. Considering $\ell = L$, the duplication-limited constraint $\bar{L}>\frac{2}{H_2(\p)}$ from before stays the same. But now for $\ell = 0$ we require only 
$$c=\frac GN = \lam \inv < \bar L\,,$$ 
  The obvious necessary condition of Section~\ref{sec:lower} that the genome be covered is evidently sufficient as well. 






==> converse_intuitive.tex <==
\section{Upper Bound}
\label{sec:lower}


In this section we derive an information theoretic upper bound on the capacity for the i.i.d. sequence model; such a bound holds for any algorithm, even one possessing unbounded computational power. The bound is made up of two necessary conditions. First, reconstruction of the DNA sequence is clearly impossible if it is not covered by the reads . Second, reconstruction is not possible if there are excessively long duplicated portions of the genome. Loosely, such duplications (which arise due to the random nature of the DNA source) create confusion if they are longer than the read length. 

The rest of this section examines these necessary conditions in more detail, determining which choices of parameters cause them not to be satisfied.

\subsection{Coverage}
In order to reconstruct the DNA sequence it is necessary to observe each of the nucleotides, i.e. the reads must cover the sequence (see Figure~\ref{fig:coverage}). Worse than the missing nucleotides, a gap in coverage also creates ambiguity in the order of the contiguous pieces.
The paper of Lander and Waterman \cite{} studied the coverage problem in the context of DNA sequencing, while the basic coverage condition was first obtained in \cite{}. 

\begin{figure}
\begin{center}
%\includegraphics[width=6.5in]{figures/Coverage.eps} 
\end{center}
\caption{The reads must cover the sequence.}
\label{fig:coverage}
\end{figure}

A standard coupon collector-style argument gives the following bound. 
\begin{theorem}[Coverage-limited]
Suppose the sequencing rate is $c=\frac GN\geq \bar{L} $. Then the sequence is not covered by the reads with probability $1-o(1)$. This implies that $C(\bar{L})\leq \bar{L}$. 
\end{theorem}
\begin{proof}
\texttt{Include proof?}
\end{proof}

Coverage depends on the location of the reads but is independent of the DNA sequence itself. Switching focus to the DNA sequence, we next study the duplication condition.

\subsection{Duplication}
The random nature of the DNA sequence gives rise to a variety of patterns. 
The key observation is that the existence of one such pattern, consisting of two pairs of interleaved duplications of length at least equal to the read length $L$, precludes reconstruction.  In this situation, two different DNA sequences are consistent with the observed set of reads and no number of reads can remove the ambiguity (see Figure~\ref{fig:duplication}). 

\begin{figure}
\begin{center}
%\includegraphics[width=6.5in]{figures/Duplication.eps} 
\end{center}
\caption{Two pairs of interleaved duplications create ambiguity.}
\label{fig:duplication}
\end{figure}

Following Arratia et al. \cite{}, the first-order question is how many duplications of length $L$ are expected to arise. If there are two pairs of interleaved duplications, then there must be some duplications in the first place; and conversely, if there are several pairs of duplications, it is plausible that with a reasonably high probability they will be interleaved. 
 Denoting by $\s_i^L$ the length-$L$ subsequence starting at position $i$, we have 
 \begin{equation}\label{e:expectedDuplicates1}
 \E[\text{\# of length $L$ duplications}] = \sum_{1\leq i<j\leq G} \P(\s_i^L=\s_j^L)\,.
 \end{equation}
 Now, the probability that two specific \emph{disjoint} length-$L$ subsequences are identical is given by a simple computation, recorded in the following lemma.
\begin{lemma}\label{l:matchProb}
Let $X^\ell=(X_{1},X_{2},\dots,X_{\ell})$ and $Y^\ell=(Y_{1},Y_{2},\dots,Y_{\ell})$ with $X_{i},Y_i\sim \p$ be two independent length-$\ell$ sequences of i.i.d. random variables with distribution $\p$.
Then  $$\P(X^\ell=Y^\ell)=\Big(\sum_i p_i^2\Big)^\ell= e^{-\ell H_2(\p)}\,,$$ 
where $H_2(\p)=-\log \big(\sum_i p_i^2\big)$ is the R\'enyi entropy of order two.
\end{lemma}
 Ignoring terms in \eqref{e:expectedDuplicates1} where $\s_i^L$ and $\s_j^L$ overlap, Lemma~\ref{l:matchProb} gives
$$
\E[\text{\# of duplications}]\approx \frac{G^2}2  \,e^{-L H_2(\p)}\,.
$$
This number approaches zero, or infinity, depending on whether $\bar{L}=L/\ln G$ is greater, or less than $2/H_2(\p)$, suggesting that this is the threshold for existence of interleaved duplications. 
Arratia et al. \cite{} carried out a thorough analysis of randomly occurring duplications for the same i.i.d. sequence model as ours, and our Theorem~\ref{t:duplication} confirming $2/H_2(\p)$ as the threshold is a special case of their Theorem~???. 
\begin{theorem}[Duplication-limited]\label{t:duplication}
If $\bar{L} < \frac2{H_2(\mathbf{p})}$, then a random DNA sequence contains two pairs of interleaved duplications with probability $1-o(1)$ and hence $C(\bar{L})=0$. 
\end{theorem}

\texttt{A simple proof of this can be achieved by considering $G/L$ disjoint substrings, then computing the probability of two pairs of duplications, and noting by a coupling argument that with probability 1/2 they are interleaved.}



==> extension_repeats.tex <==
\subsection{Repeats}
\label{subsec:repeats}



The Markov model captures small spatial scale correlations in the DNA sequence. However, it does not capture the large-scale repetitive nature of DNA sequences: It is known that approximately half of human DNA is composed of repetitions with lengths of the order of hundreds to 20,000 base pairs \cite{}. From the discussion of Section~\ref{sec:formulation} we know that if contiguous reads are used, a prohibitively long read length, at least the length of the repeats, is necessary to bridge the repeats. More generally, repeats are understood to be one of the main bottlenecks for assembly \cite{}.

With this in mind, we study in this section a simple repeat model, where a length-$K$ sequence $\x$ is selected i.i.d. according to the distribution $\p=(p_1,p_2,p_3,p_4)$, and then $M$ copies of $\x$ are equally spaced within the DNA sequence. We denote by $G_0$ the length of the original DNA sequence, with $G=G_0+MK$ the total length after adding in the repeats. It turns out that it is meaningful to scale the number of repeats as $M=G^\al$, and we define the normalized repeat length $\bar{K}= K / \ln G$.

Most sequencing platforms attempt to overcome the difficulty imposed by repeats by using so-called \emph{paired-end reads}; here, the reads come in pairs with a (approximately) known separation. The basic physical sequencing model we consider in this section produces $N/2$ pairs of reads of length-$L$, with each pair having a separation of $J$ bases (see Figure~\ref{fig:matePairs}). The normalized read separation is $\bar J:= J/\ln G$. Note that if $J=0$ the model reduces to the single-read model with $N/2$ total reads and read length $2L$. The total length $I=2L+J$ is often called the \emph{insert length}. 

\begin{figure}
\begin{center}
\includegraphics[width=3in]{figures/PairedEndReads.eps}
\end{center}
\caption{Paired-end reads. The read separation is $J$, with each mate-pair having length $L$, for a total length $I=2L+J$.}
\label{fig:matePairs}
\end{figure}

%Fix this paragraph
As a corollary to the main result of this section, we show that with paired-end reads the required read length $L$ is not significantly affected by introducing repeats. Specifically, under some natural assumptions on the parameters, it suffices to have a read separation of $\bar J=\bar K+4\al/H_2(\p)$ in order to recover the original capacity region. The repeats do not degrade performance at all as long as the read separation is a little larger than the size of the repeat.
\begin{corollary}\label{c:MatePairsRecon}
If the normalized read separation satisfies $\bar J> \bar{K}+4\al/H_2(\p)$, then the capacity of the i.i.d. model is achievable, i.e. the repeats do not degrade performance.
\end{corollary}

One might initially guess that having a read separation $J$ larger than the repeat length $K$ would suffice in the above corollary. This is not the case, however, due to the random symbols \emph{adjacent} to the repeats: there will actually be duplications of length approximately $K+ 2\al/H_2(\p)$ in the DNA sequence.

A general sufficient condition for reconstruction, implying Corollary~\ref{c:MatePairsRecon}, is as follows. 

\begin{theorem}[Repeats]\label{t:repeats}
Suppose $\bar{L}>2/H_2(\p)$, $R< \bar{L}$, and ??? conditions on $K$, $M$, $G$: $K\geq L$,. Then all rates $R< \al\inv\bar L + \al\inv \frac1{2}[\bar{J}-(4\alpha/H_2(\p) + \bar K)]$ are achievable.
\end{theorem}

The algorithm achieving the rates in Theorem~\ref{t:repeats} is a modification of the Greedy Algorithm described in Section~\ref{sec:formulation}. It first assembles contiguous stretches (contigs) between the repeats using the individual reads, and then uses the mate-pair information to place the contigs in the correct order.
%Recall that the weight $w_{ij}=w(r_i,r_j)$ between two reads $r_i$ and $r_j$ is defined to be the length of the longest matching suffix of $r_i$ and prefix of $r_j$. In this section we use the modified weight $\w_{ij}:=w_{ij}-w(r_i,\x)$, which is defined such that the overlap between $r_i$ and the repeat $\x$ does not count toward the weight (see Figure~\ref{fig:modWeight}).

The analysis showing that the contigs between repeats can be assembled is technically more difficult than that for the basic greedy algorithm, but is intuitively similar. We therefore focus here on the second objective, ordering the contigs using the mate-pair information. The proofs are deferred to Section~\ref{}.


We say that a mate-pair \emph{bridges} a repeat if at least $d$ nucleotides of the left-read extend to the left of the repeat and $d$ nucleotides of the right-read extend to the right of the repeat (see Figure~\ref{fig:simpleBridge}). The parameter $d$ is chosen sufficiently large so that for each bridged repeat, the contigs on either side can be uniquely determined, thus giving their relative position. If all repeats are bridged, and $d$ is indeed sufficiently large, then we can order the contigs. 

We now heuristically compute for which rates $R$ every repeat is bridged with high probability. As illustrated in Figure~\ref{fig:simpleBridge}, for each repeat there is an interval of length $J+2L-(2d+K)$ such that if the left-endpoint of the left-read in a mate-pair is located in the interval, then the repeat is bridged. Note that \emph{left-reads} have an arrival rate of $\lam/2$ (where $\lam=N/G$ as before). Thus the probability that a particular repeat is not bridged is approximately $e^{-\lam(2L+J-(2d+K))/2}$. The expected number of non-bridged repeats is
$$
Me^{-\lam(2L+J-(2d+K))/2}\,,
$$
and this number approaches zero if 
$$
R=\lam\inv < \frac{L+\frac12[J-(2d+K)]}{\ln M}
$$
or equivalently
$$
R< \al\inv\bar L + \al\inv \frac1{2}[\bar{J}-(2\bar d + \bar K)]\,,
$$
where $\bar d = d/\ln G$.

It is not enough for each repeat to have a bridging mate-pair: such a mate-pair must uniquely determine the contigs on either side. It turns out that if the parameter $d$ is sufficiently large, this is possible. Let us assume that if a mate-pair bridges a repeat, then it can be correctly positioned relative to the repeat. In this case, if each length-$d$ subsequence immediately preceding a repeat is unique, and the same holds for each length-$d$ subsequence immediately following a repeat, then a bridging mate-pair can be identified with unique contigs. 

We compute the expected value of duplications among length-$d$ subsequences immediately preceding a repeat, 
$$
M\left(\sum p_i^2\right)^d\,,
$$
and this quantity approaches zero if $d> \frac{2\ln M}{H_2(\p)}$ or equivalently 
$$\bar d=\frac{d}{\ln G}> \frac{2\al}{H_2(\p)}\,.$$ The same argument applies to the subsequences following repeats, suggesting that this value for $d$ is sufficient. 



\begin{figure}
\centering
\vspace{-0.5cm}
\includegraphics[width=5in]{figures/SimpleRepeatBridge.eps}
%\vspace{-0.5cm}
\caption{A mate-pair bridges a repeat if the left-read arrives in an interval of length $J+2L-(2d+K)$.}
\label{fig:simpleBridge}
\end{figure}



Slightly modifying the necessary conditions of Section~\ref{sec:formulation} shows that the achievable rate of Theorem~\ref{t:repeats} is nearly optimal.

\begin{proposition}[Paired-end coverage-limited]
A rate $R<\bar{L}$ is necessary in order to cover the genome. Since the gap in coverage is located in a uniformly random position, this implies $C(\bar{L}) \leq \bar{L}$.
\end{proposition}

The following necessary condition on the insert length $I=2L+J$ comes by noting that performance would not decrease if we had single (long) reads of length $I$ instead of each paired-end reads, since one could just ignore the subsequence within each such long read corresponding to the gap between mate-pairs.

\begin{proposition}[Paired-end duplication-limited]
With probability $1-o(1)$ there will be interleaved repeats of length at least $K+2\ln M/H_2(\p)$, and thus an insert length $I>K+2\ln M/H_2(\p)$ is necessary for reconstruction.
\end{proposition}

\begin{figure}
\centering
\begin{pspicture}(-1,-1)(5,5)
%\psgrid[gridwidth=.03,griddots=5,subgridwidth=.02,subgriddiv=2,subgriddots=5]
\psline{->}(0,0)(5,0)
\psline{->}(0,0)(0,5)
\pscustom[linecolor=red,linewidth=.05]{
\psplot[plotpoints=200]
{1.25}{4.5}{x}% cos(40 x) / 2
}
\psline[linecolor=blue,linewidth=.1](0,0)(1.25,0)
\psline[linecolor=red,linewidth=.05](0,0)(1.25,0)
\rput[r](-.1,4.8){$R$}
\rput[t](4.8,-.1){$\bar L $}
\rput[t](1.25,-.1){$2\over H_2(\mathbf{p})$}
\rput[r](-.1,1.25){$2 \over H_2(\mathbf{p})$}
\rput(3.7,4.4){$ C( \bar L)$}
\psline[linecolor=red,linestyle=dashed](1.25,0)(1.25,1.25)
\psline[linecolor=blue,linewidth=.1](1.25,0.25)(4.5,3.5)
\end{pspicture}
%% a straight plot of C(\bar{L}) vs \ba{L}. No regimes. No G/N on y-axis.
\caption{Plot of the sequencing capacity $C$ as a function of the normalized read length~$\bar{L}$.}
\label{fig:plot_repeats}
\end{figure}














==> information.tex <==
\section{Information}

\label{sec:information}

\begin{theorem}\label{t:information}
The mutual information rate is $I(R)=R$ for any value of $\bar{L}>2/H_2(\p)$. 
\end{theorem}

\texttt{Question: What is the mutual information rate for $0<\bar{L}<2/H_2(\p)$?} \\

Let's assume $H(X)=G$, i.e. the nucleotides are uniformly distributed, and let $\De= \bar{L}-\frac{2}{H_2(\mathbf{p})}>0$. ($H_2(\mathbf{p})=1$, so $\De = \bar{L} - 1$.) 

\begin{enumerate}
\item Use the \emph{sequential} algorithm to merge reads down to a minimum overlap of $ \bar{\ell}^* = 1+\De/2$.  
\item Note that with probability $1-o(1)$ no two reads will be confused at overlap $\bar{\ell}^* = (1+\De/2) \log G$. This is exactly the Lander-Waterman value of $T$ which gives no false positives. 
\item \emph{Allow $N^\al$ contigs for $\al<1$}. By Stirling's approximation, the number of bits required to resolve the ambiguity in the ordering of the contigs  is approximately $\ln[(N^{\al})!]= O(N^\al\ln N)=o(N)$. By Lemma 1 below, there are $N^{1-\lam(\bar{L}-\bar{\ell}^*)} = N^{1-\lam\De/2} $ contigs.
\item \emph{There are $o(N)$ uncovered nucleotides.} Each nucleotide is \emph{not} covered with probability $(1-\bar{L})^N$, and so the expected number of uncovered nucleotides is $G(1-\bar{L})^N$, which is exponentially smaller than $N$, and the actual number of uncovered nucleotides is reasonably well-concentrated. 
\item By items 2 and 3, recovering the true sequence from our partial reconstruction requires only $o(N)$ bits.   This implies (by mutual information chain rule) that $I(X;R_1,\dots, R_N)= H(X)-o_N(1)$, or $I(R)=\frac GN=R$ \emph{for any value of $\bar{L}>1$}. In other words, $C(\bar{L})=\infty$ for $\bar{L}>1$!
\end{enumerate}


\begin{lemma}
The number of contigs, restricting to read overlaps of at least $\ell^*$, is approximately $Ne^{-\lam(L-\ell^*)}=e^{\ln N(1-\lam(\bar{L}-\bar{\ell}^*))}=N^{1-\lam(\bar{L}-\bar{\ell}^*)}$.  
\end{lemma}




==> related_work.tex <==
This is for related works.

==> repeats_proofs.tex <==


\section{Proofs for repeats}

\newcommand{\Vt}{{\widetilde V}}
\newcommand{\Ut}{{\widetilde U}}
\newcommand{\AAt}{{\widetilde \calA}}


 \paragraph{\underline{Repeats Algorithm:}}
\begin{enumerate}
\item Find the repeated $K$-mer $\x$.
\item Construct modified read overlap graph.
\item Run greedy algorithm to assemble contigs
\item Order contigs using mate-pair information
\end{enumerate}



%%
%% describe why J>K does not suffice
%% step 5 is confusing

\begin{proof}[Proof of Theorem~\ref{t:repeats}]
We now describe each step of the algorithm and prove correctness. We assume $L\geq (1+2\eps) 2/H_2(\p)$, for some $\eps>0$.
\paragraph{Step 1: Find repeated $K$-mer.}\

\emph{Input:} Set of reads $\RR$. 

\emph{Output:} Subsequence $\x$ of the repeated $K$-mer. \\
%The probability that a particular $L$-mer appears multiple times is at least $(1-\frac1G)^{N-1}\approx e^{-\lam}$.
%Define $\eps>0$ such that $L=(1+2\eps)2/H_2(\p)$ and let $L_0:=(1+\eps)2\ln G/H_2(\p)$. Denote by $\a$ the initial length-$L$ subsequence of $\x$. We first argue that we can find $\a$. To begin, consider the set of all $L_0$-mers within the reads. Select an $L_0$-mer which is repeated, \emph{except for the first symbol differing}. We claim that this $L_0$-mer, minus the first symbol, contains of the first $L_0-1$ symbols from $\x$. 
%To verify this, note that 

\paragraph{Step 2: Construct modified read overlap graph $\G$.}\ \\
 \emph{Input:} Set of reads $\RR$ and repeated $K$-mer $\x$. \\
 \emph{Output:} Modified read overlap graph $\G$. 

 
Let $\a$ and $\b$ represent the first and last $L$-mers, respectively, in the repeat $\x$. We start with the standard read overlap graph $\G$, which has one node representing each read, and modify it by adding two special nodes, one node labeled $\a$ and another node labeled $\b$. Outgoing edges are removed from node $\a$ and incoming edges are removed from node $\b$. Nodes $\a$ and $\b$ are permanent, in the sense that the greedy algorithm does not remove edges from these nodes. Additionally, all nodes except $\a$ and $\b$ corresponding to reads entirely contained in the repeat $\x$ are removed. The weight $W_{ij}$ on each edge $e_{ij}$ represents the length of the longest suffix of $\bR_i$ identical to a prefix of $\bR_j$ (as before).

%The algorithm will construct paths $\hat\PP_i=(\b,\bR_{i_1},\bR_{i_2},\dots,\bR_{i_k},\a)$ and from each such path produce a reconstructed contig $\hat \bC_i$ by aligning the reads.


\paragraph{Step 3: Run greedy algorithm to reconstruct contigs.}\ \\
 \emph{Input:} Modified read overlap graph $\G$. \\
\emph{Output:} Set of estimated contigs $\{\hat \bC_1,\dots, \hat \bC_M\}$. %paths $\hat\PP_i=(\b,\bR_{j_1},\bR_{j_2},\dots,\bR_{j_{k_i}},\a)$.  

Here $\bC_i$ is the $i$th contig between copies of $\x$. We run the greedy algorithm, merging reads until no edges remain in the graph $\G$. The result is a set of contigs $\{\hat \bC_1,\dots, \hat \bC_M\}$, each starting with $\b$ and ending with $\a$. Let $\EE$ be the error event, that the set of estimated contigs does not equal the true set of contigs. 

The analysis resembles that for the original Greedy Algorithm, but the details are different. The main issue is that it is nearly impossible to identify the successor of a read significantly overlapping a copy of $\x$; fortunately, merging one read which overlaps $\x$ to another read overlapping $\x$ does not actually lead to an error in the reconstructed sequence, assuming they are aligned correctly, and thus the distinction is in the definition of the error events.

In order to define the error events, we consider separately the subset of \emph{interior} reads $\RRi$ which overlap a copy of the repeat $\x$ by at most $2\eps \ln G/H_2(\p)$, the subset of \emph{right border} reads $\RRbr$, which overlap from the left a copy of $\x$ by more than $2\eps \ln G/H_2(\p)$, and the subset of \emph{left border} reads $\RRbr$ which overlap from the right a copy of $\x$, again by more than $2\eps \ln G/H_2(\p)$. %We add $\a$ to the set $\RRbr$ and $\b$ to $\RRbl$. 
The set of border reads is denoted $\RRb=\RRbl\cup\RRbr$. For each left border read $\bR_i$ we let $\Vt_i$ denote the amount of physical overlap with the repeat $\x$, and similarly we let $\Ut_i$ denote the physical overlap of the repeat $\x$ with a right border read.

Let $\EE_1$ denote the event that an interior read is merged incorrectly, either as predecessor or successor. As before, this includes merging to the read's valid successor but at the wrong relative position as well as merging to an impostor.
Let $\EE_2$ be the event that one border read is merged to another border read at the wrong position \emph{relative} to the repeat. $\EE_3$ denotes the event that a border read is merged to either $\a$ or $\b$ with an incorrect offset. 
Finally, $\EE_4$ is the event that the DNA sequence is not covered by the reads. 
\begin{claim}
The error event is contained as $\EE\subseteq \EE_1\cup \EE_2\cup \EE_3\cup \EE_4$.
\end{claim}

\begin{lemma}
If $\lam \bar L> 1$, then the DNA sequence fails to be covered by the reads with probability $\P(\EE_4)=o(1)$. 
\end{lemma}
\begin{proof}
The proof is almost the same as for contiguous reads. Each nucleotide in the DNA sequence has probability $\left(1 - \frac{2L}G \right)^{N/2}$ of not being covered, so taking a union bound over the $G$ nucleotides gives
$$
\P(\EE_3)\leq G \left(1 - \frac{2L}G \right)^{N/2} \leq \exp\{\ln G - \lam L\}=o(1)
$$
if $\lam \bar L>1$.
\end{proof}

We now turn to $\P(\EE_1)$. Similarly to the discussion preceding \eqref{e:Adecomb}, we may write $\EE_1=\cup_\ell \calA_\ell$, where now $\calA_\ell$ is the event that the first error in merging \emph{to an interior read} occurs at stage $\ell$.
We have 
\begin{equation}
\calA_\ell \subseteq \BB_{\ell}\cup \CC_{\ell}\,,
\end{equation}
where  $\BB_\ell$ and $\CC_\ell$ are defined using the shorthand $\II_i=\{\bR_i\in \RRi\}$ as
\begin{align}
\BB_\ell  &\triangleq \{\bR_j\neq \bR_i^s, U_j\leq \ell, V_i\leq \ell, W_{ij}=\ell \mbox{ for some $i \not = j$}\}\cap(\II_i\cup \II_j) 
\label{eq:eventB}\\
\CC_\ell & \triangleq  \{\bR_j=\bR_i^s, U_j=V_i< \ell, W_{ij}=\ell \mbox{ for some $i \not = j$}\} \cap(\II_i\cup \II_j)\,. 
\end{align}

\begin{lemma}
If $\bar{L}>2/H_2(\p)$ and $\lam \bar{L}>1$, then $\P(\EE_1)=o(1)$.
\end{lemma}
\begin{proof}
The proof is essentially identical to that of Theorem~\ref{p:IIDachievability}, but uses the modified definitions of the events $\BB_\ell $ and $\CC_\ell$. 
\end{proof}

We next bound $\P(\EE_2\cap \EE_1^c)$; it turns out to be easier to work with $\EE_2\cap \EE_1^c$ than $\EE_2$ alone. We write $\EE_2=\cup_\ell \AAt_\ell$, where $\AAt_\ell$ is the event that the first error in merging two border reads occurs at stage $\ell$. As discussed above, such an error occurs if the reads are merged at the wrong offset \emph{relative to the repeat}, but two reads may be merged without error even if they are not adjacent. Here $\bR_j$ is offset $\Ut_j-\Ut_i$ nucleotides from $\bR_i$ relative to the repeat, while if if they are merged at stage $\ell$ then $W_{ij}=\ell$ and their offset is $L-W_{ij}$. Thus
\begin{equation}\label{e:error2event}
\AAt_\ell\cap \EE_1^c \subseteq \{ \Ut_j-\Ut_i\neq L-W_{ij}, V_i\leq \ell, U_j\leq \ell, W_{ij}=\ell, \text{ for some } i\neq j \} \cap (\II_i^c\cap \II_j^c)\,.
\end{equation}
The justification for \eqref{e:error2event} involves one subtlety. If $\AAt_\ell\cap \EE_1^c$ occurs, then some pair of reads $\bR_i, \bR_j\in \RRb$ has $W_{ij}=\ell$, and since they are merged erroneously, it must be the case that $\Ut_j-\Ut_i\neq L-W_{ij}$. Now, if $V_i>\ell$, there are two cases: either $\bR_i^s\in \RRi$ or $\bR_i^s\in \RRb$. The first case cannot occur as it would result in an error in merging $\bR_i^s$, violating our restriction to $\EE_1^c$. For the second case, 

\begin{lemma}
If $\bar{L}>2/H_2(\p)$, then $\P(\EE_2)=o(1)$.
\end{lemma}
\begin{proof} To begin, define
\begin{equation}
\DD^{ij}_\ell = \{ \Ut_j-\Ut_i\neq L-W_{ij}, V_i\leq \ell, U_j\leq \ell, W_{ij}=\ell \} \cap (\II_i^c\cap \II_j^c)\,,
\end{equation}
so that 
$$\AAt_\ell\cap \EE_1^c\subseteq \cup_{i\neq j} \DD^{ij}_\ell\,,$$
and by the union bound $\P(\AAt_\ell\cap \EE_1^c )\leq N^2 \P(\DD^{12}_\ell)$.
\end{proof}


\paragraph{Step 4: Order contigs using mate pair information.}
%We first describe a simple method of ordering the contigs, analogous to the sequential assembly algorithm described in subsection~\ref{subsec:sequential}, which obtains any rate satisfying the bounds $R<\bar{L}$ and $R<\frac{\log G}{\log M}\bar{L}+\frac1{\log M}[J-(K+4\log M/H_2(\p))]$. This rate is lower than that of Theorem~\ref{t:repeats}, with the $-2/H_2(\p)$ term multiplied by two. The second method of ordering the contigs is analogous to the greedy algorithm of subsection~\ref{sec:achieve}, and obtains the rate ???.
We assume that the input to Step~4 consists of $M$ random contigs, each of length $G_0/M$, and $N/2$ randomly located pairs of reads; the goal is to find the correct order of the contigs. The ordering algorithm for Step 4 is described as follows, with the parameter $d=(1+\eps)2\ln M / H_2(\p)$.
\begin{enumerate}
\item Take an arbitrary contig $\bC$. Find a left-read $\bR$ consistent with starting in a position at most $J+2L-(2d+K)$, and at least $d$, bases from the right end of $\bC$.
\item Find a contig $\bC'$ consistent with the right-read $\bR'$ being located in a position at least $d$, but no more than $J+2L-(2d+K)$, bases from the left end. Form a new contig by concatenating $\bC, \x, \bC'$.
\end{enumerate}





We say that a mate-pair \emph{bridges} a repeat if at least $d$ nucleotides of the left-read extend to the left of the repeat and $d$ nucleotides of the right-read extend to the right of the repeat. If every repeat has a mate-pair bridging it, then to ensure correctness of the algorithm it must only be checked that identifying reads with contigs is done correctly.
The error event may thus be decomposed as $\EE\subseteq \EE_{\text{bridge}}\cup\EE_{\text{ident}}$, where
\begin{align}
\EE_\text{bridge}&=\{\text{there is a repeat without a bridging mate-pair}\} \\
\EE_\text{ident}&=\{\text{a read is identified incorrectly}\}\,.
\end{align}

\begin{lemma}\label{c:pairedReadPos}
If $R<\frac{1}{2\ln M}[J+2L-(2d+K)]$, then $\P(\EE_\text{bridge})=o(1)$.
\end{lemma}
\begin{proof}
A repeat is bridged if there is a left-read whose left end lies in an interval of size $J+2L-(2d+K)$ (see Figure~\ref{fig:simpleBridge}). Thus, the probability a particular repeat is not bridged by any of the $N/2$ mate-pairs is $\big(1-\frac{J+2L-(2d+K)}{G}\big)^{N/2}$, and applying the union bound to the $M$ repeats gives
$$
\P(\EE_\text{bridge})\leq M\Big(1-\frac{J+2L-(2d+K)}{G}\Big)^{N/2}\leq M e^{-\frac{\lam}{2} [J+2L-(2d+K)]}\,,
$$ where $\lam:=N/G=R\inv$. Plugging in the hypothesis of the lemma completes the proof.
\end{proof}

We now turn to bounding $\EE_\text{ident}$.
\begin{lemma}
If $\bar{L}>2/H_2(\p)$, then  $\P(\EE_\text{ident})=o(1)$.
\end{lemma}
\begin{proof}
We will prove that in Step~1 left-reads are correctly identified with contigs, and by symmetry of the arguments, the desired result will hold for right-reads as well.

An error in identifying a left-read $\bR$ to a contig $\bC$ occurs only if $\bR$ is consistent with starting in a position $\ell$ bases from the right of $\bC$, where $d\leq \ell \leq J+2L-(2d+K)$, but does not actually overlap $\bC$ at all. Rephrasing in terms of the DNA sequence $\s$ itself, the error event satisfies $\EE_\text{ident}\subseteq \UU$, where $\UU$ is the event that some length-$L$ subsequence from $\s$, starting $d\leq \ell \leq J+2L-(2d+K)$ bases from the end of a contig, appears elsewhere in a position disjoint from the contig.

The event $\UU$ may be decomposed as $\UU\subseteq \cup_{d\leq \ell \leq L}\UU_\ell$, with
\begin{align*}
\UU_\ell = \{\text{a }&\text{length-$L$ subsequence, overlapping a contig by $\ell$ bases,}\\ &\text{is repeated in a subsequence disjoint from the contig}\}\,.
\end{align*}
The event $\UU_L$ implies that two mutually independent length-$L$ i.i.d. sequences with distribution $\p$ are equal. An application of the union bound over the at most $G^2$ possible pairs of length-$L$ sequences gives
$$
\P(\UU_L)\leq G^2 e^{-LH_2(\p)}=o(1)\,,
$$ where the second step is by the assumption $\bar{L}> 2/H_2(\p)$.

Next, we show that $\P(\cup_{d\leq \ell<L}\UU_\ell)=o(1)$. First, $\UU_\ell= \WW_\ell\cup \VV_\ell$, where we define $\WW_\ell$ to be the event that a length-$L$ subsequence, overlapping a contig by $\ell$ bases, is repeated strictly within some other contig, and $\VV_\ell$ to be the event that a length-$L$ subsequence, overlapping a contig by $\ell$ bases, is equal to a length-$L$ subsequence overlapping a repeat by at least one base (and disjoint from the contig).

The event $\WW_\ell$ implies that two independent length-$L$ subsequences are equal, of which there are at most $MLG$ such pairs; the union bound thus gives $\P(\WW_\ell)\leq MLG e^{-L H_2(\p)}$. In contrast, there are at most $(ML)^2$ pairs of length-$L$ subsequences both touching a repeat, and $\VV_\ell$ implies that two independent length-$\ell$ subsequences are equal, so $\P(\VV_\ell)\leq (ML)^2 e^{-\ell H_2(\p)}\leq (ML)^2 e^{-dH_2(\p)}$.

Applying the union bound yet again, we have
$$
\P(\cup_{d\leq \ell<L}\UU_\ell) \leq \sum_{\ell=1}^{L-1} [\P(\WW_\ell)+\P(\VV_\ell)]\leq ML^2G e^{-L H_2(\p)} + M^2 L^3 e^{-dH_2(\p)}= o(1)\,.
$$
The lemma is proved, since $\EE_p\subseteq \big(\cup_{d\leq \ell<L} \UU_\ell \big)\bigcup \UU_L$.
\end{proof}




\end{proof}



